AI Choreographer: Music Conditioned 3D Dance Generation with AIST++

We present AIST++, a new multi-modal dataset of 3D dance motion and music, along with FACT, a Full-Attention Cross-modal Transformer network for generating 3D dance motion conditioned on music. The proposed AIST++ dataset contains 5.2 hours of 3D dance motion in 1408 sequences, covering 10 dance genres with multi-view videos with known camera poses -- the largest dataset of this kind to our knowledge. We show that naively applying sequence models such as transformers to this dataset for the task of music conditioned 3D motion generation does not produce satisfactory 3D motion that is well correlated with the input music. We overcome these shortcomings by introducing key changes in its architecture design and supervision: FACT model involves a deep cross-modal transformer block with full-attention that is trained to predict $N$ future motions. We empirically show that these changes are key factors in generating long sequences of realistic dance motion that are well-attuned to the input music. We conduct extensive experiments on AIST++ with user studies, where our method outperforms recent state-of-the-art methods both qualitatively and quantitatively.

==> figures/aist_pipeline.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{figs/aist_pipeline.jpg}
\caption{\textbf{AIST++ Dataset Construction Pipeline.} Given the AIST multi-view dance videos dataset, we proposed a reconstruction pipeline that can reliably reconstruct the 3D motion without manually labeling the 2D keypoints or body shape segmentation.}
\label{fig:aist_pipeline}
\vspace{-3mm}
\end{figure*}


==> figures/aist_reproj_error.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{figs/aist_reproj_error.png}
\caption{\textbf{AIST++ 3D Keypoints Re-projection Error Distribution.} We compare the average pixel distance of the re-projected 2D keypoints and the detected 2D keypoints~\cite{papandreou2017towards} for each video on 1920x1080 resolution.}
\label{fig:aist_reproj_error}
\vspace{-3mm}
\end{figure}

==> figures/genre_correlation.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{figs/genre_correlation.png}
\caption{\textbf{Correlations between generated motions conditioned on different genre of musics.} The generated motions have a clear distribution difference conditioned on different genre of musics.
}
\label{fig:genre_correlation}
\vspace{-3mm}
\end{figure}

==> figures/teaser.tex <==
\begin{figure*}
\centering
\includegraphics[width=1.0\textwidth]{figs/teaser.pdf}
\caption{\textbf{Learning to Generate 3D Dance with Our AIST++ Dataset.} We present our AIST++ dataset and a multi-modal transformer-based network architecture for training a computational model that learns to output 3D dance choreography conditioned on music. 
}
\label{fig:teaser}
\end{figure*}


==> tables/dataset_stats.tex <==
\begin{table*}[t]
\centering{
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}[c]{ccccccc}
\hline
Genres & Musics & Music Tempo & Motions & Choreographs & Motion Duration (sec.) & Total Seconds  \\
\hline
ballet jazz & 6 & 80 - 130 & 141 & \multirow{10}{6em}{85\% basic + 15\% advanced} & 7.4 - 12.0 basic / 29.5 - 48.0 adv. & 1910.8 \\
street jazz & 6 & 80 - 130 & 141 &  & 7.4 - 12.0 basic / 14.9 - 48.0 adv. & 1875.3 \\
krump & 6 & 80 - 130 & 141 &  & 7.4 - 12.0 basic / 29.5 - 48.0 adv. & 1904.3 \\
house & 6 & 110 - 135 & 141 &  & 7.1 - 8.7 basic / 28.4 - 34.9 adv. & 1607.6 \\
LA-style hip-hop & 6 & 80 - 130 & 141 &  & 7.4 - 12.0 basic / 29.5 - 48.0 adv. & 1935.8 \\
middle hip-hop & 6 & 80 - 130 & 141 &  & 7.4 - 12.0 basic / 29.5 - 48.0 adv. & 1934.0 \\
waack & 6 & 80 - 130 & 140 &  & 7.4 - 12.0 basic / 29.5 - 48.0 adv. & 1897.1 \\
lock & 6 & 80 - 130 & 141 &  & 7.4 - 12.0 basic / 29.5 - 48.0 adv. & 1898.5 \\
pop & 6 & 80 - 130 & 140 &  & 7.4 - 12.0 basic / 29.5 - 48.0 adv. & 1872.9 \\
break & 6 & 80 - 130 & 141 &  & 7.4 - 12.0 basic / 23.8 - 48.0 adv. & 1858.3 \\
\hline
total & 60 & & 1408 &  &  & 18694.6
\end{tabular}}}
\caption{AIST++ Dataset. We reconstruct these subset of AIST Dataset that are single-person dance sequences}
\label{tab:dataset_stats}
\vspace{-3mm}
\end{table*}
